Parallel Cluster-BFS and Applications to Shortest Paths

Breadth-first Search (BFS) is one of the most important graph processing subroutines, especially for computing the unweighted distance. Many applications may require running BFS from multiple sources. Sequentially, when running BFS on a cluster of nearby vertices, a known optimization is using bit-parallelism. Given a subset of vertices with size $k$ and the distance between any pair of them is no more than $d$, BFS can be applied to all of them in total work $O(dm(k/w+1))$, where $w$ is the length of a word in bits and $m$ is the number of edges. We will refer to this approach as cluster-BFS (C-BFS). Such an approach has been studied and shown effective both in theory and in practice in the sequential setting. However, it remains unknown how this can be combined with thread-level parallelism. In this paper, we focus on designing efficient parallel C-BFS based on BFS to answer unweighted distance queries. Our solution combines the strengths of bit-level parallelism and thread-level parallelism, and achieves significant speedup over the plain sequential solution. We also apply our algorithm to real-world applications. In particular, we identified another application (landmark-labeling for the approximate distance oracle) that can take advantage of parallel C-BFS. Under the same memory budget, our new solution improves accuracy and/or time on all the 18 tested graphs.

==> figs_algs/alg_LL_cluster.tex <==
\begin{algorithm}[t]
  \small
 \caption{Framework of Landmark Labeling with Clusters\label{alg:ClusterLL}}
%  \KwIn{A graph $G=(V,E)$ and a list of clusters landmarks $S_i\in S$}
 \SetKwFor{parForEach}{parallel\_for\_each}{do}{endfor}
 \SetKwInOut{Maintains}{Maintains}
 \DontPrintSemicolon
 \myfunc{\textsc{Construct\_Index}$(G, S)$ \tcp*[f]{$G=(V,E)$, $S$ are landmarks}}{
  $\delta[\cdot][\cdot]$ \tcp*[f]{A 2D array of size $n\times |S|$, $\delta[v][i]$ stores the \compactdis between vertex $v$ and cluster $C_i\in S$.}\\
  \tcp{$\delta[v][i]$ stores a triple $\langle S_0, S_1, \delta_{\min}\rangle$}
  \For{$i\gets 0 ,\dots, |S|-1$}{
    $\delta_i^T[1,\cdots,n] \gets \textsc{\ccbfs}(G,C_i)$\\
    \For{$v\in V$}{
      $\delta[v][i]\gets \delta_i^T[v]$
    }
  }
  \Return $\delta$
 }
 \myfunc{\textsc{Query}$(u,v)$}{
  $\delta_{uv}\gets\infty$\\
  \For{$i\gets 0,\dots, |S|-1$}{
    $\delta_{tmp} \gets \delta[u][i].\delta_{\min}+\delta[v][i].\delta_{\min}$\\
    \If {$\delta[u][i].S_0 \cap \delta[u][i].S_0 \neq \emptyset$}{
      $\delta_{tmp} \gets \delta_{tmp}-2$
    }\ElseIf{$\delta[u][i].S_0 \cap \delta[u][i].S_1 \neq \emptyset$ or $\delta[u][i].S_1 \cap \delta[u][i].S_0 \neq \emptyset$}{
      $\delta_{tmp} \gets \delta_{tmp}-1$
    }
    $\delta_{uv} \gets \min(\delta_{uv}, \delta_{tmp})$
  }
  \Return $\delta_{uv}$
 }
\end{algorithm} 

==> figs_algs/alg_prunedBFS.tex <==
\begin{algorithm}[t]
  \small
 \caption{Framework of Pruned BFS\label{alg:PrunedBFS}}
%  \KwIn{A graph $G=(V,E)$ and an order of vertices $\{v_1, \cdots, v_n\}$}
%  \KwOut{The index $L$}
 % \SetKwFor{parForEach}{parallel\_for\_each}{do}{endfor}
 % \SetKwInOut{Maintains}{Maintains}
 \DontPrintSemicolon
 \myfunc{\textsc{Construct\_Index}$(G, \{v_1,\cdots,v_n\})$}{
  \tcp{The inputs are a graph $G$, and an vertex order $\{v1,\dots, v_n\}$}
 $L[v]\gets \emptyset$ for $\forall v\in V$ \tcp*[f]{$L$ is the index we will construct}\\
 \For{$i\gets 1,\dots, n$}{
    $Q\gets $ a queue with only one element $v_i$\\
    $\delta(v_i)\gets 0$ and $\delta(v)\gets \infty, \forall v\in V\setminus{v_i}$\\
    \While{$Q \neq \emptyset$}{
      $u\gets Q.pop()$\\
      \tcp{$Query(v_i,u,L)$ answers the distance using the current $L$}
      \If{$Query(v_i,u,L)\leq \delta(u)$}
      {
        continue \tcp*[f]{Pruned}
      }
      $L[u]\gets L[u]\cup \{(v_i, \delta(u))\}$\\
      \For{$v\in N(u)$}{
        \If{$\delta(v)=\infty$}
        {$\delta(v)$ $\gets$ $\delta(u)+1$ \\
        $Q.push(v)$
        }
      }
    }
 }
 \Return $L$
 }
%  \myfunc{Query$(u,v)$}{
%   \tcp{Note that the labels in $L(v)$ are sorted by the input orders}
%   $it_u\gets L(u).begin()$ \tcp*[f]{$it_u$ and $it_v$ are iterators for $L(v)$ and $L(u)$}\\
%   $it_v\gets L(v).begin()$\\
%   $\delta_{uv}\gets \infty$
%   \While{$it_u \neq L(u).end()$ or $it_v \neq L(v).end()$}{
%     \If{}
%   }
%  }
\end{algorithm} 

==> figs_algs/table0.tex <==
\begin{tabular}{l|rrl}\toprule
  \textbf{Dataset} &\textbf{n} &\textbf{m} &\textbf{Notes} \\\midrule
  EP &75,879 &811,480 &Epinions1~\cite{backstrom2006group} \\
  SLDT &77,360 &938,360 &Slashdot~\cite{leskovec2009community} \\
  ND &325,729 &1,514,730 &NotreDame~\cite{nr} \\
  DBLP &317,080 &2,099,732 &DBLP~\cite{yang2015defining} \\
  YT &1,134,890 &5,975,248 &com-youtube~\cite{yang2015defining} \\
  Wiki &2,394,384 &9,319,129 &WikiTalk~\cite{nr} \\
  SK &1,694,616 &22,188,418 &skitter~\cite{nr, skitter} \\
  IN04 &1,382,908 &27,560,356 & in\_2004~\cite{BoVWFI,Boldi-2011-layered} \\
  FL &1,715,254 &31,110,081 &flickr~\cite{nr,mislove2008growth} \\
  LJ &4,847,571 &85,702,474 &soc-LiveJournal1~\cite{backstrom2006group} \\
  HW &1,069,126 &112,613,306 &hollywood\_2009~\cite{nr,BoVWFI} \\
  FBUU &58,790,782 &184,416,390 &socfb-uci-uni~\cite{nr,traud2012social,red2011comparing,siamr} \\
  FBKN &59,216,214 &185,044,024 &socfb-konect~\cite{nr,traud2012social,red2011comparing,siamr} \\
  OK &3,072,627 &234,370,166 &com-orkut~\cite{yang2015defining} \\
  INDO &7,414,866 &301,969,638 &indochina~\cite{nr,Boldi-2011-layered,boldi2004-ubicrawler} \\
  EU &11,264,052 &521,886,106 &eu-2015-host~\cite{BoVWFI,Boldi-2011-layered,MSB} \\
  UK &18,520,486 &523,574,516 &uk-2002~\cite{BoVWFI,Boldi-2011-layered} \\
  AR &22,744,080 &1,107,806,146 &arabic~\cite{BoVWFI,Boldi-2011-layered} \\
  TW &41,652,231 &2,405,026,092 &Twitter~\cite{kwak2010twitter} \\
  FT &65,608,366 &3,612,134,270 &Friendster~\cite{yang2015defining} \\
  SD &89,247,739 &3,880,015,728 &sd\_arc~\cite{webgraph} \\
  \bottomrule
  \end{tabular}

==> figs_algs/table1.tex <==
\begin{tabular}{>{\bf}l@{ }|ccl|c|@{ }c@{  }c@{  }c@{ }|c@{  }c}
  \toprule
          & \multicolumn{3}{c|}{Graph Information} & Seq-BFS & \multicolumn{3}{c|}{
          Spd., relative to previous
          } &\multicolumn{2}{c}{ \BatchBFS} \\
  Dataset &                 $n$ &     $m$ &                                                          Notes & Time(s) &       +EdgeMap &     +Cluster &    +parallel &  Spd.       & Time(s) \\
\midrule
     EP &             75.9K &  811K &                         Epinions1~\cite{backstrom2006group} &    0.19 &                      0.92$\times$ & 10.8$\times$ & 9.41$\times$ &        93.2$\times$ &   0.002 \\
   SLDT &             77.4K &  938K &                       Slashdot~\cite{leskovec2009community} &    0.21 &                      1.13$\times$ & 8.12$\times$ & 12.3$\times$ &         112$\times$ &   0.002 \\
     ND &              325K & 1.51M &                                         NotreDame~\cite{nr} &    0.34 &                      0.27$\times$ & 19.0$\times$ & 15.6$\times$ &        79.5$\times$ &   0.004 \\
   DBLP &              317K & 2.10M &                                DBLP~\cite{yang2015defining} &    0.77 &                      0.61$\times$ & 15.4$\times$ & 20.8$\times$ &         194$\times$ &   0.004 \\
     YT &             1.13M & 5.98M &                         com-youtube~\cite{yang2015defining} &    3.30 &                      0.87$\times$ & 13.3$\times$ & 35.7$\times$ &         411$\times$ &   0.008 \\
   Wiki &             2.39M & 9.32M &                                          WikiTalk~\cite{nr} &    9.22 &                      1.59$\times$ & 12.5$\times$ & 44.6$\times$ &         885$\times$ &   0.010 \\
     SK &             1.69M & 22.2M &                                  skitter~\cite{nr, skitter} &    6.56 &                      1.14$\times$ & 10.7$\times$ & 39.7$\times$ &         480$\times$ &   0.014 \\
   IN04 &             1.38M & 27.6M &                   in\_2004~\cite{BoVWFI,Boldi-2011-layered} &    4.08 &                      0.39$\times$ & 22.3$\times$ & 19.3$\times$ &         169$\times$ &   0.024 \\
     FL &             1.72M & 31.1M &                          flickr~\cite{nr,mislove2008growth} &    9.06 &                      1.39$\times$ & 9.71$\times$ & 40.8$\times$ &         553$\times$ &   0.016 \\
     LJ &             4.85M & 85.7M &                  soc-LiveJournal1~\cite{backstrom2006group} &    39.8 &                      1.30$\times$ & 11.5$\times$ & 55.2$\times$ &         820$\times$ &   0.049 \\
     HW &             1.07M &  112M &                            hollywood\_2009~\cite{nr,BoVWFI} &    18.7 &                      2.77$\times$ & 6.61$\times$ & 47.3$\times$ &         864$\times$ &   0.022 \\
   FBUU &             58.8M &  184M &    socfb-uci-uni~\cite{nr,traud2012social,red2011comparing} &     268 &                      0.91$\times$ & 17.1$\times$ & 63.4$\times$ &         985$\times$ &   0.273 \\
   FBKN &             59.2M &  185M &     socfb-konect~\cite{nr,traud2012social,red2011comparing} &     176 &                      0.73$\times$ & 16.3$\times$ & 62.4$\times$ &         741$\times$ &   0.238 \\
     OK &             3.07M &  234M &                           com-orkut~\cite{yang2015defining} &    61.6 &                      2.09$\times$ & 5.96$\times$ & 64.3$\times$ &         801$\times$ &   0.077 \\
   INDO &             7.41M &  301M & indochina~\cite{nr,Boldi-2011-layered,boldi2004-ubicrawler} &    38.8 &                      0.48$\times$ & 23.5$\times$ & 38.1$\times$ &         433$\times$ &   0.090 \\
     EU &             11.3M &  521M &          eu-2015-host~\cite{BoVWFI,Boldi-2011-layered,BMSB} &     119 &                      1.44$\times$ & 12.9$\times$ & 43.6$\times$ &         808$\times$ &   0.148 \\
     UK &             18.5M &  523M &                    uk-2002~\cite{BoVWFI,Boldi-2011-layered} &    91.8 &                      0.73$\times$ & 18.6$\times$ & 50.2$\times$ &         679$\times$ &   0.135 \\
     AR &             22.7M & 1.11B &                     arabic~\cite{BoVWFI,Boldi-2011-layered} &     147 &                      0.59$\times$ & 21.6$\times$ & 37.0$\times$ &         474$\times$ &   0.310 \\
     TW &             41.7M & 2.41B &                             Twitter~\cite{kwak2010twitter}  &     723 &                      2.93$\times$ & 5.22$\times$ & 55.0$\times$ &         841$\times$ &   0.859 \\
     FT &             65.6M & 3.61B &                          Friendster~\cite{yang2015defining} &    1673 &                      2.41$\times$ & 6.46$\times$ & 61.6$\times$ &         958$\times$ &   1.745 \\
     SD &             89.2M & 3.88B &                                     sd\_arc~\cite{webgraph} &    1504 &                      1.11$\times$ & 16.4$\times$ & 62.1$\times$ &        1130$\times$ &   1.332 \\
\midrule
GeoMean &                   &       &                                                             &    22.2 &                      1.03$\times$ & 12.3$\times$ & 36.9$\times$ &         467$\times$ &   0.047 \\
\bottomrule
\end{tabular}


==> figs_algs/table_pll.tex <==
\begin{tabular}{l|c|rr|r|rr|rr|c|c}
\toprule
&  & \multicolumn{2}{c|}{avg. \# normal labels} &    \multicolumn{1}{c|}{Index} & \multicolumn{2}{c|}{CCBFS time} & \multicolumn{2}{c|}{Pruned BFS time} & Total Index & Total Query \\
Dataset & \# Clusters &             baseline & OURS & Size(GB) &    OURS(s) &    speedup &         OURS(s) &    speedup &     Time(s) &    Time(ms) \\
\midrule
   Wiki &         16 &                   34 &   35 &      1.0 &       0.27 & 18$\times$ &             8.2 &  6$\times$ &           9 &         1.1 \\
     SK &         64 &                  123 &  126 &      2.7 &       1.05 & 31$\times$ &            15.0 & 18$\times$ &          16 &         4.2 \\
     FL &         64 &                  268 &  270 &      3.9 &       1.02 & 40$\times$ &            24.0 & 25$\times$ &          25 &         4.8 \\
     HW &         64 &                 2237 & 2281 &     12.4 &       1.26 & 82$\times$ &           302.6 & 36$\times$ &         304 &        23.2 \\
   INDO &         64 &                  323 &  349 &     19.6 &       5.62 & 44$\times$ &           421.4 &  9$\times$ &         428 &         5.3 \\
     EU &         64 &                    - &  945 &     61.0 &       9.92 &          - &          1384.5 &          - &        1396 &         9.3 \\
     LJ &        512 &                    - & 2585 &     97.7 &      22.97 &          - &          2718.1 &          - &        2742 &        28.4 \\
\bottomrule
\end{tabular}

